Where and How to Enhance: Discovering Bit-Width Contribution for Mixed Precision Quantization

Mixed precision quantization (MPQ) is an effective quantization approach to achieve accuracy-complexity trade-off of neural network, through assigning different bit-widths to network activations and weights in each layer. The typical way of existing MPQ methods is to optimize quantization policies (i.e., bit-width allocation) in a gradient descent manner, termed as Differentiable (DMPQ). At the end of the search, the bit-width associated to the quantization parameters which has the largest value will be selected to form the final mixed precision quantization policy, with the implicit assumption that the values of quantization parameters reflect the operation contribution to the accuracy improvement. While much has been discussed about the MPQ improvement, the bit-width selection process has received little attention. We study this problem and argue that the magnitude of quantization parameters does not necessarily reflect the actual contribution of the bit-width to the task performance. Then, we propose a Shapley-based MPQ (SMPQ) method, which measures the bit-width operation direct contribution on the MPQ task. To reduce computation cost, a Monte Carlo sampling-based approximation strategy is proposed for Shapley computation. Extensive experiments on mainstream benchmarks demonstrate that our SMPQ consistently achieves state-of-the-art performance than gradient-based competitors.

==> sec/0_abstract.tex <==
\begin{abstract}
Mixed precision quantization (MPQ) is an effective quantization approach to reduce the size and computational overhead of neural network, through constraining different bit-widths of network weights and activations in different layers. The typical way of existing MPQ methods is to optimize quantization policies (i.e., bit-width assignments) with gradient descent, termed as differentiable MPQ (DMPQ). At the end of the search, the bit-width operations with the largest parameter magnitudes will be selected to form the final mixed precision quantization policy, with the implicit assumption that the values of quantization parameters reflect the operation contribution to the accuracy improvement. While much has been discussed about the MPQ’s improvement, the bit-width selection process has received little attention. We study this problem and show that the magnitude of quantization parameters does not necessarily reflect the actual contribution of the bit-width to the task performance. We propose a Shapley-based MPQ method, which measures the bit-width operation’s direct contribution on the MPQ task. We evaluate the proposed method and find that it is able to consistently achieve better accuracy than gradient-based counterparts. Furthermore, we find that it also performs more efficiently than its comparators on a set of datasets and several search spaces.
\end{abstract}

